Envy Freedom and Prior-free Mechanism Design

We consider the provision of an abstract service to single-dimensional agents. Our model includes position auctions, single-minded combinatorial auctions, and constrained matching markets. When the agents' values are drawn from a distribution, the Bayesian optimal mechanism is given by Myerson (1981) as a virtual-surplus optimizer. We develop a framework for prior-free mechanism design and analysis. A good mechanism in our framework approximates the optimal mechanism for the distribution if there is a distribution; moreover, when there is no distribution this mechanism still performs well. We define and characterize optimal envy-free outcomes in symmetric single-dimensional environments. Our characterization mirrors Myerson's theory. Furthermore, unlike in mechanism design where there is no point-wise optimal mechanism, there is always a point-wise optimal envy-free outcome. Envy-free outcomes and incentive-compatible mechanisms are similar in structure and performance. We therefore use the optimal envy-free revenue as a benchmark for measuring the performance of a prior-free mechanism. A good mechanism is one that approximates the envy free benchmark on any profile of agent values. We show that good mechanisms exist, and in particular, a natural generalization of the random sampling auction of Goldberg et al. (2001) is a constant approximation.

==> multi-unit-benchmarks.tex <==
\subsection{Refined Analysis for Multi-Unit Auctions}

% A PICTURE OF THE ALLOCATION FUNCTION WITH SHADED PAYMENT WOULD BE
% GREAT TO INCLUDE HERE!


 %~ \begin{figure*}[ht]
 %~ \begin{center}
 %~ \includegraphics[scale=.7]{allocation}
 %~ \end{center}
 %~ \caption{The allocation function $\alloci(\vali)$ for $\vals_{-i}$ fixed. The area of the shaded region is the payment $\pricei(\vali)$ specified by Lemma~\ref{l:ic}.}
 %~ \label{fig.allocation}
 %~ \end{figure*}
Now consider repeating the above discussion but with the empirical
distribution $\dist$ for valuation profile $\vals$.  We could sell $k$
units at price $\valith[k]$.  Denote this revenue by
$$
R(k) = k \valith[k].
$$ Again, $\IR(k)$ is the concave hull of $R(k)$.

We could then pick an $i$ and $j$ with $i < k < j \leq n$ and make the
following offer to this particular set of agents with profile $\vals$:
high-valued agents with values in $[\valith[i], \infty)$ win for sure
  and low-valued agents with values in $[\valith[j],\valith[i])$ win
    with probability given by the ratio between the number of units
    left and the number of agents on the interval (i.e., by {\em
      lottery}).  The payments for such an allocation rule are given
    by Lemma~\ref{l:ic}: low-valued agents pay $\valith[j]$ and
    high-valued agents pay $\valith[i] - \frac{(\valith[i] -
      \valith[j])(k-i+1)}{j-i+1}$.  Notice that to calculate the
    high-valued agent payments one must note that a high-valued agent
    might try to bid as if they were low-valued, this would result in
    one fewer units being claimed by high-valued agents which means
    there are $k-i+1$ units to be randomly allocated among the
    remaining $j-i+1$ agents (see Figure~\ref{fig.allocation}).  Let $\rhat_{i,j}(k)$ denote the total
    resulting revenue from this approach.  Notice that $\rhat_{i,j}(k) \neq
      \R_{i,j}(k)$.





As described in the preceding section the Bayesian optimal auction
divides valuation space into intervals of equal priority.  For the
purpose of maximizing profit one would only want to use intervals
bounded by agent valuations, i.e., of the form
$[\valith[j],\valith[i])$, as this would have all winners paying the
  maximum possible.  This and the above discussion gives intuition for
  the following lemma.

\begin{lemma} \label{lem.HR} \cite{HR-08} $\bm(k,\vals) = \sup_{i,j} \rhat_{i,j}(k,\vals)$ and
  $\bm^{(2)}(k,\vals) = \sup_{i,j \geq 2} \rhat_{i,j}(k,\vals)$.
\end{lemma}

$\bm$ will be tough for us to work with so we use the following
definition which (as the theorem below shows) provides a good upper
bound.

\begin{definition}
$\fbar(k,\vals) = \max_{i\leq k}\IR(i,\vals)$ and
$\fbartwo(k,\vals) = \max_{2\leq i\leq k}\IR(i,\vals)$.
\end{definition}

The following theorem relates $\bm$, $\f$, and $\fbar$.  This will be
used later in our proof to relate conceptually easier bounds in terms
of $\fbar$ with our desired bound in terms of $\bm$. Also, the argument $\vals$ in
the above benchmarks will be dropped when it is clear from the context.

\begin{theorem}\label{thm.benchmarks} For all valuations, $\vals$,\\
  \begin{enumerate}
  \item $\f(k,\vals) \leq \g(k,\vals) \leq \fbar(k,\vals)$.
Similarly $\ftwo(k,\vals) \leq \gtwo(k,\vals) \leq \fbartwo(k,\vals)$.
\item $\fbar(k,\vals) \leq 2 \f(k,\vals)$.
There exists $\vals$ such that $\g(k,\vals) = (2-\tfrac{1}{k})\f(k,\vals)$.
\item  $ \fbar(k,\vals) \leq \min \{ \tfrac{4}{3}, 1+\tfrac{1}{k} \} \g(k,\vals)$.
  \end{enumerate}
\end{theorem}

\begin{proof} We prove each part separately.
\begin{enumerate}
\item
The first part of the theorem follows almost immediately from the definitions and
Lemma \ref{lem.HR}.


 \begin{figure*}[htbp]
 \begin{center}
 \includegraphics[scale=.7]{pics/benchmarks}
 \end{center}
 \caption{Illustration for proof of Theorem~\ref{thm.benchmarks}.}
 \label{fig.benchmarks}
 \end{figure*}


\item For the second part, recall that $\IR$ is concave.  If $\IR$
  attains its maximum before the supply runs out, that is $\fbar(k) =
  R(l)$ for some $l\leq k$, then the lemma follows trivially since
  $\fbar(k) = \f(k)$.  So suppose not. Then $\IR$ is monotonically
  non-decreasing in the interval $[1,k]$ and hence $\fbar(k) =
  \IR(k)$.  Suppose $\IR(k)$ is on the line joining $R(i)$ and
  $R(j)$, where $i< k < j$. Then
\begin{eqnarray*}
\IR(k) &=& \tfrac{1}{j-i} \left( (k-i) R(j) + (j-k)R(i)\right )\\
& =& R(i) + \tfrac{k-i}{j-i}(R(j) - R(i)) \text{  (segment AB in Figure \ref{fig.benchmarks})}\\
&\leq & R(i) + \tfrac{k}{j} R(j) \text{  (segment CD in Figure \ref{fig.benchmarks})}\\
& \leq & R(i) + R(k) \leq 2 \f(k).
\end{eqnarray*}
The first inequality on the last line follows since
$$\tfrac{k}{j} R(j)= \tfrac{k}{j} j \valith[j] = k \valith[j] \leq k
\valith[k] = R(k).$$

The above bound is almost tight.  Let $\vali[1] = k$, $\vali[2]=\vali[3] = \cdots = \vali[n] = 1.$
Then $\f(k) = k$, where as $\g(k) = \rhat_{1,k}(k) = k + (k-1)(1 - \tfrac{k}{n}) $
which tends to $2k-1$ as $n$ tends to infinity.



% \begin{lemma}
%  $ \fbar(k) \leq \tfrac{4}{3} \g(k)$.
% \end{lemma}
% \begin{proof}
\item For the third part, again, the interesting case is when
  $\fbar(k) = \IR(k)$, and
\[ \IR(k) = \tfrac{1}{j-i} \left( (k-i) R(j) + (j-k)R(i)\right ).\]
Let $p=\valith[i]$ and $q=\valith[j]$ and define
\[\rhat(k)  = \rhat_{i,j}(k) = (k-i)q + i \left( p - \tfrac{(p-q)(k-i+1)}{j-i+1} \right ) .\]
In the interval $[i,j]$, $\rhat$ is a linear function of $k$ with
$\rhat(i) = i \left( p - \tfrac{p-q}{j-i+1} \right )$ and slope
$\tfrac{q(j+1) - ip}{j-i+1}$.
In comparison, in the same interval,
$\IR$ is a linear function of $k$ with $\IR(i) = ip $ and slope
$\tfrac{qj - ip}{j-i}$.  $\IR(i) > \rhat(i)$ where as the slope of
$\rhat$ is higher than $\IR$.  Hence the minimum ratio of $\rhat(k)$
to $\IR(k)$ occurs at $k=i$, and $\IR(i) - \rhat(i) =
\tfrac{i(p-q)}{j-i+1}$ which is clearly less than $\tfrac{ip}{4}$ if
$j-i \geq3$.
(In Figure \ref{fig.benchmarks}, ratio of segment EF to EG is 1:j-i+1.)
Also, $j-i$ is at least 2, since $i< k < j$.  So we are
only left with the case when $j-i =2$.  In this case we use the fact
that $R(j)\geq R(i)$, which follows from the definition of
$\IR$. This implies $(i+2)q \geq ip$, which in turn implies that
$\tfrac{i(p-q)}{j-i+1}$ is less than $\tfrac{ip}{4}$ by simple
algebra.  In any case, we have that $\IR(i)\leq \tfrac{4}{3} \rhat(i)$
and in turn $\fbar(k) \leq \tfrac{4}{3}\g(k)$.

Again, using the fact that $R(j)\geq R(i)$, we get that
$\tfrac{i(p-q)}{j-i+1}$ is less than $\tfrac{q(j-i)}{j-i+1}\leq q$.
Further note that $qk \leq \g(k)$ since $qk$ is the revenue of the
posted price auction with price $q$.  Thus $\IR(i) - \rhat(i)$, and in
fact, $\IR(k) - \rhat(k)$ is less than $\g(k)/k$ for all $k \in
[i,j]$. Thus, $\fbar(k) \leq \left( 1 + \tfrac{1}{k}\right) \g(k)$.
\end{enumerate}
\end{proof}

\paragraph*{Remark}
It immediately follows from the above theorem that any algorithm that
is an $\alpha$-approximation to $\f$ is a $2\alpha$-approximation to
$\fbar$.  Currently the best known auction is from Hartline and
McGrew~\cite{HM-05} and achieves an approximation factor of 3.25 to
$\f$.  Thus, it is a 6.5 approximation to $\fbar$.  We do not manage
to prove that RSEM is better than this; however, there is no reason to
believe that it is not.



==> multi-unit.tex <==
\section{Refined Analysis for Multi-Unit Auctions}

\subsection{The optimal Bayesian optimal benchmark}
% A PICTURE OF THE ALLOCATION FUNCTION WITH SHADED PAYMENT WOULD BE
% GREAT TO INCLUDE HERE!


 %~ \begin{figure*}[ht]
 %~ \begin{center}
 %~ \includegraphics[scale=.7]{allocation}
 %~ \end{center}
 %~ \caption{The allocation function $\alloci(\vali)$ for $\vals_{-i}$ fixed. The area of the shaded region is the payment $\pricei(\vali)$ specified by Lemma~\ref{l:ic}.}
 %~ \label{fig.allocation}
 %~ \end{figure*}
Now consider repeating the above discussion but with the empirical
distribution $\dist$ for valuation profile $\vals$.  We could sell $k$
units at price $\valith[k]$.  Denote this revenue by
$$
R(k) = k \valith[k].
$$ Again, $\IR(k)$ is the concave hull of $R(k)$.

We could then pick an $i$ and $j$ with $i < k < j \leq n$ and make the
following offer to this particular set of agents with profile $\vals$:
high-valued agents with values in $[\valith[i], \infty)$ win for sure
  and low-valued agents with values in $[\valith[j],\valith[i])$ win
    with probability given by the ratio between the number of units
    left and the number of agents on the interval (i.e., by {\em
      lottery}).  The payments for such an allocation rule are given
    by Lemma~\ref{l:ic}: low-valued agents pay $\valith[j]$ and
    high-valued agents pay $\valith[i] - \frac{(\valith[i] -
      \valith[j])(k-i+1)}{j-i+1}$.  Notice that to calculate the
    high-valued agent payments one must note that a high-valued agent
    might try to bid as if they were low-valued, this would result in
    one fewer units being claimed by high-valued agents which means
    there are $k-i+1$ units to be randomly allocated among the
    remaining $j-i+1$ agents (see Figure~\ref{fig.allocation}).  Let $\rhat_{i,j}(k)$ denote the total
    resulting revenue from this approach.  Notice that $\rhat_{i,j}(k) \neq
      \R_{i,j}(k)$.





As described in the preceding section the Bayesian optimal auction
divides valuation space into intervals of equal priority.  For the
purpose of maximizing profit one would only want to use intervals
bounded by agent valuations, i.e., of the form
$[\valith[j],\valith[i])$, as this would have all winners paying the
  maximum possible.  This and the above discussion gives intuition for
  the following lemma.

\begin{lemma} \label{lem.HR} \cite{HR-08} $\bm(k,\vals) = \sup_{i,j} \rhat_{i,j}(k,\vals)$ and
  $\bm^{(2)}(k,\vals) = \sup_{i,j \geq 2} \rhat_{i,j}(k,\vals)$.
\end{lemma}

$\bm$ will be tough for us to work with so we use the following
definition which (as the theorem below shows) provides a good upper
bound.

\begin{definition}
$\fbar(k,\vals) = \max_{i\leq k}\IR(i,\vals)$ and
$\fbartwo(k,\vals) = \max_{2\leq i\leq k}\IR(i,\vals)$.
\end{definition}

The following theorem relates $\bm$, $\f$, and $\fbar$.  This will be
used later in our proof to relate conceptually easier bounds in terms
of $\fbar$ with our desired bound in terms of $\bm$. Also, the argument $\vals$ in
the above benchmarks will be dropped when it is clear from the context.

\begin{theorem}\label{thm.benchmarks} For all valuations, $\vals$,\\
  \begin{enumerate}
  \item $\f(k,\vals) \leq \g(k,\vals) \leq \fbar(k,\vals)$.
Similarly $\ftwo(k,\vals) \leq \gtwo(k,\vals) \leq \fbartwo(k,\vals)$.
\item $\fbar(k,\vals) \leq 2 \f(k,\vals)$.
There exists $\vals$ such that $\g(k,\vals) = (2-\tfrac{1}{k})\f(k,\vals)$.
\item  $ \fbar(k,\vals) \leq \min \{ \tfrac{4}{3}, 1+\tfrac{1}{k} \} \g(k,\vals)$.
  \end{enumerate}
\end{theorem}

\begin{proof} We prove each part separately.
\begin{enumerate}
\item
The first part of the theorem follows almost immediately from the definitions and
Lemma \ref{lem.HR}.


 \begin{figure*}[htbp]
 \begin{center}
 \includegraphics[scale=.7]{pics/benchmarks}
 \end{center}
 \caption{Illustration for proof of Theorem~\ref{thm.benchmarks}.}
 \label{fig.benchmarks}
 \end{figure*}


\item For the second part, recall that $\IR$ is concave.  If $\IR$
  attains its maximum before the supply runs out, that is $\fbar(k) =
  R(l)$ for some $l\leq k$, then the lemma follows trivially since
  $\fbar(k) = \f(k)$.  So suppose not. Then $\IR$ is monotonically
  non-decreasing in the interval $[1,k]$ and hence $\fbar(k) =
  \IR(k)$.  Suppose $\IR(k)$ is on the line joining $R(i)$ and
  $R(j)$, where $i< k < j$. Then
\begin{eqnarray*}
\IR(k) &=& \tfrac{1}{j-i} \left( (k-i) R(j) + (j-k)R(i)\right )\\
& =& R(i) + \tfrac{k-i}{j-i}(R(j) - R(i)) \text{  (segment AB in Figure \ref{fig.benchmarks})}\\
&\leq & R(i) + \tfrac{k}{j} R(j) \text{  (segment CD in Figure \ref{fig.benchmarks})}\\
& \leq & R(i) + R(k) \leq 2 \f(k).
\end{eqnarray*}
The first inequality on the last line follows since
$$\tfrac{k}{j} R(j)= \tfrac{k}{j} j \valith[j] = k \valith[j] \leq k
\valith[k] = R(k).$$

The above bound is almost tight.  Let $\vali[1] = k$, $\vali[2]=\vali[3] = \cdots = \vali[n] = 1.$
Then $\f(k) = k$, where as $\g(k) = \rhat_{1,k}(k) = k + (k-1)(1 - \tfrac{k}{n}) $
which tends to $2k-1$ as $n$ tends to infinity.



% \begin{lemma}
%  $ \fbar(k) \leq \tfrac{4}{3} \g(k)$.
% \end{lemma}
% \begin{proof}
\item For the third part, again, the interesting case is when
  $\fbar(k) = \IR(k)$, and
\[ \IR(k) = \tfrac{1}{j-i} \left( (k-i) R(j) + (j-k)R(i)\right ).\]
Let $p=\valith[i]$ and $q=\valith[j]$ and define
\[\rhat(k)  = \rhat_{i,j}(k) = (k-i)q + i \left( p - \tfrac{(p-q)(k-i+1)}{j-i+1} \right ) .\]
In the interval $[i,j]$, $\rhat$ is a linear function of $k$ with
$\rhat(i) = i \left( p - \tfrac{p-q}{j-i+1} \right )$ and slope
$\tfrac{q(j+1) - ip}{j-i+1}$.
In comparison, in the same interval,
$\IR$ is a linear function of $k$ with $\IR(i) = ip $ and slope
$\tfrac{qj - ip}{j-i}$.  $\IR(i) > \rhat(i)$ where as the slope of
$\rhat$ is higher than $\IR$.  Hence the minimum ratio of $\rhat(k)$
to $\IR(k)$ occurs at $k=i$, and $\IR(i) - \rhat(i) =
\tfrac{i(p-q)}{j-i+1}$ which is clearly less than $\tfrac{ip}{4}$ if
$j-i \geq3$.
(In Figure \ref{fig.benchmarks}, ratio of segment EF to EG is 1:j-i+1.)
Also, $j-i$ is at least 2, since $i< k < j$.  So we are
only left with the case when $j-i =2$.  In this case we use the fact
that $R(j)\geq R(i)$, which follows from the definition of
$\IR$. This implies $(i+2)q \geq ip$, which in turn implies that
$\tfrac{i(p-q)}{j-i+1}$ is less than $\tfrac{ip}{4}$ by simple
algebra.  In any case, we have that $\IR(i)\leq \tfrac{4}{3} \rhat(i)$
and in turn $\fbar(k) \leq \tfrac{4}{3}\g(k)$.

Again, using the fact that $R(j)\geq R(i)$, we get that
$\tfrac{i(p-q)}{j-i+1}$ is less than $\tfrac{q(j-i)}{j-i+1}\leq q$.
Further note that $qk \leq \g(k)$ since $qk$ is the revenue of the
posted price auction with price $q$.  Thus $\IR(i) - \rhat(i)$, and in
fact, $\IR(k) - \rhat(k)$ is less than $\g(k)/k$ for all $k \in
[i,j]$. Thus, $\fbar(k) \leq \left( 1 + \tfrac{1}{k}\right) \g(k)$.
\end{enumerate}
\end{proof}

\paragraph*{Remark}
It immediately follows from the above theorem that any algorithm that
is an $\alpha$-approximation to $\f$ is a $2\alpha$-approximation to
$\fbar$.  Currently the best known auction is from Hartline and
McGrew~\cite{HM-05} and achieves an approximation factor of 3.25 to
$\f$.  Thus, it is a 6.5 approximation to $\fbar$.  We do not manage
to prove that RSEM is better than this; however, there is no reason to
believe that it is not.


\pagebreak
\subsection{The Myerson auction for empirical distributions}

The random sampling auction we wish to analyze runs the Myerson
auction on a partition of the agents with distribution given
empirically by the opposite partition.  We now explicitly describe
what $\mye{\dist}$ does when $\dist$ is the empirical distribution for
valuation profile $\vals$.  Recall that Myerson's auction for a
distribution simply allocates the $k$ units to the agents with highest
priority breaking ties in priority randomly.  Of course, the key
property of Myerson's auction is that it partitions valuation space
into intervals of equal priority in the optimal way.  From our
preceding discussion this partitioning is given by looking at the
revenue function $R(\cdot)$ and its concave hull $\IR(\cdot)$.
Intervals where theses functions are not equal form a priority class.
Specifically, let $i_1 \leq \cdots \leq i_T$ index the $T$ agents $i$
satisfying $R(i) = \IR(i)$ on the rising slope of $\IR(\cdot)$
(i.e., $i_T = \arg\max_i R(i)$).  The equal-priority intervals are
\[[\valith[i_T], \valith[i_{T-1}]],
(\valith[i_{T-1}],\valith[i_{T-2}]],\ldots,(\valith[2],\valith[1]],(\valith[1],\infty).\]
  Agents with values below the smallest interval, i.e., strictly less
  than $\valith[i_T]$ are rejected.


The set of bidders is partitioned into sets $A$ and $B$.  Let the bids
in $A$ be $\valith[1]^A \geq \valith[2]^A \geq \ldots$ and so on.  Let
$\dist^A$ be the empirical distribution from bidders in $A$ and
consider running the Myerson auction with this distribution on the
bidders in $B$, i.e., $\mye{\dist^A}(\vals^B)$.  Myerson allocates as follows.  Let $i^A_1 < i^A_2 < \cdots < i^A_T $ be the indices of
agents on the concave hull of the revenue curve for $\dist^A$ (as
described in the preceding paragraph).  Let $p^A_t =
\valith[i^A_t]^A$.  The equal priority intervals are
$$[p^A_{T},p^A_{T-1}],(p^A_{T-1},p^A_{T-2}], \ldots,(p^A_{2},p_{1}],
  (p^A_{1},\infty).$$ The bidders in $B$ are allocated odd-numbered
  items.  Let $j^B_t = |\{l \in B : \valith[l]^B \geq p_t^A \}|$.  Now
  if $\tfrac{k}{2} \in [j^B_t,j^B_{t+1})$, then the top $j^B_t$ always
    get the item and pay $p^A_t - \tfrac{p_t^A - p_{t+1}^A}{j^B_{t+1}
      - j^B_t +1}$.  Bidders with values in the interval
    $(p_{t+1}^A,p_t^A]$ win remaining units at price $p_{t+1}^A$ with ties broken randomly.

\subsection{The performance of the random sampling auction}

 \begin{figure*}[htbp]
  \begin{center}
  \includegraphics[scale=.8]{pics/revenuecurves}
  \end{center}
  \caption{Revenue curves illustrated for the proof of Lemma~\ref{lem.swap}.}
 \label{fig.revcurves}
  \end{figure*}


Our analysis of the performance of the RSEM auction
uses a lemma from the recent paper of \cite{AMS-09} that analyses the RSOP auction
for unlimited supply.
They prove a lemma about the expectation of a certain random variable, let's call it $X$, that is
used to lower bound the revenue of the RSOP auction.
We show that the same quantity $X$ can be used to bound the revenue of the RSEM auction
for limited supply as well.
While the fact that $X$ lower bounds the revenue of the RSOP auction for unlimited supply
is more or less straightforward, the analogous statement for the RSEM auction for limited supply
is more complicated because the revenue of lotteries is  more complicated
that the revenue of posted price auctions.

We now define the random variable $X$.
Without loss of generality, let the highest bidder be in $B$.
Let $s_i = \left|\{ j \in A :  \vali[j] \geq \valith \}\right|$
be the number of bidders in $A$ among the top $i$ bidders.
Note that the distribution of $s_i$ is independent of the actual values,
and has the same distribution as the following  discrete random walk on integers:
for each $i$, $s_i$ is either $s_{i-1}$, or $s_{i-1} +1$,
with probability half each, with $s_1= 0$.
Let $ z = \min_i {(i-s_i)/s_i}$.
Suppose that the optimum single price auction sells $\lambda$ units,
i.e.  $\ftwo = \lambda \valith[\lambda]$. Then
\[ X = z\cdot \frac{s_\lambda}{\lambda}.\]
Note that for every possible value of $\lambda$ we get a different random variable $X$.
The main lemma that we need from \cite{AMS-09} lower bounds  $\expect{X}$ for
all possible values of $\lambda$.
\begin{lemma}\label{lem.AMS}\cite{AMS-09}
For all positive integers $\lambda$,  $ \expect[]{X} \geq \frac{1}{\amscr}$.
\end{lemma}

As is usual in the analysis of random sampling auctions, we relate the
revenue of the RSEM auction from side B to some function of the values
from side A.  Here, that function is the {\em concave hull} of the
revenue curve from side A.  Let $R^A$ be the revenue curve restricted
to the bidders in $A$; more precisely $R^A(i) = i \valith^A$.  Let
$\IR^A$ be its concave hull.  However, for $i > i^A_T$, we define
$\IR^A(i) = \IR^A(i^A_T)$.  Note that this makes $\IR^A$ a
monotonically non-decreasing concave function.  Let $\RSEM(k)$ denote
the profit of the RSEM Auction with $k$ items.

\begin{lemma}\label{lem.swap}
$\RSEM(k) \geq z\IR^A(\tfrac{k}{2}) / \min\{\tfrac{4}{3}, 1 + \tfrac{1}{k} \} .$
\end{lemma}

\begin{proof}
Recall that the highest bidder is in $B$.  Define $\RSEM^B(i)$ to be the
revenue obtained by the RSEM auction from side $B$, as a function of
the number of units allocated to $B$.  In the proof we will only
consider the revenue obtained from side $B$, i.e., we will use that
$\RSEM(k) \geq \RSEM^B(k)$ .  This is tight in the worst case, because
if $\valith[1]$ is high enough, then the optimal Myerson auction for
$\dist^B$ (the empirical distribution for $B$) is to run a Vickrey
Auction with reserve price equal to $\valith[1]$. This auction would
fetch no revenue from side~$A$.

Suppose $\tfrac{k}{2} \in [j^B_t,j^B_{t+1})$.  Consider the following
  function defined on the interval $[j^B_t,j^B_{t+1})$: let $L(i)$ be
    the linear function such that $L(j_t^B)$ is equal to $j_t^Bp_t^A$
    and $L(j_{t+1}^B) = j_{t+1}^Bp_{t+1}^A$.  As in the proof of part
    3 of Theorem \ref{thm.benchmarks}, in the interval
    $[j^B_t,j^B_{t+1})$, the function $\RSEM^B(i)$ is within a factor
      $\min\{\tfrac{4}{3}, 1 + \tfrac{1}{k} \}$ of $L(i)$.  From the
      definition of $z$, we get that $j^B_t \geq zi_t^A$.  These two
      facts point to the conclusion we need.  However, the proof needs
      more argument because of the following:
\begin{itemize}
\item It could be that $L(j^B_{t+1}) < L(j^B_t)$.
We used the fact that this does not happen in the proof of Theorem \ref{thm.benchmarks}.
\item It could be that $\tfrac{k}{2} \notin [i_t^A,i_{t+1}^A)$. Thus we cannot
directly compare $L(\tfrac{k}{2})$ to $\IR^A(\tfrac{k}{2})$.
\end{itemize}


We get around these difficulties by comparing $L$ to the following function
instead. Let $\runder(z{i_t^A}) = z{i_t^A} p_t^A  $.
Extend $\runder$ to all $i \in [1,zi^A_T]$ by a linear interpolation.
For $i > zi^A_T$, let $\runder(i) = \runder(zi^A_T)$.
We note the following easy observations without proof (see Figure \ref{fig.revcurves}):
\begin{itemize}
\item For all $i$, $ \runder(zi)= z\IR^A(i)$.
\item $\runder$ is an increasing concave function.
\item For all $i \in [j^B_t,j^B_{t+1}]$, $L(i) \geq \runder(i)$.
\end{itemize}
We now argue that $L(\frac{k}{2}) \geq z\IR^A(\frac{k}{2})$ via the following
sequence of inequalities; this sequence of inequalities corresponds to the
points $A\geq B\geq C = zD$ in Figure~\ref{fig.revcurves}.
\[L(\frac{k}{2}) \geq \runder(\frac{k}{2}) \geq \runder(z\frac{k}{2})
= z\IR^A(\frac{k}{2}).\]
Therefore it is enough to show that
$$\RSEM^B(\tfrac{k}{2}) \geq L(\tfrac{k}{2}) / \min\{\tfrac{4}{3}, 1 + \tfrac{1}{k} \}.$$
The proof of this is identical\footnote{
We also have to consider an additional case, when $j^B_{t+1}-j^B_t=1$,
which is similar to the case $j^B_{t+1}-j^B_t=2$.}
to that in the proof of part 3 of Theorem \ref{thm.benchmarks},
unless  $L(j^B_{t+1}) < L(j^B_t)$.
In case $L(j^B_{t+1}) < L(j^B_t)$,
we use the observation that the revenue of the auction actually
decreases in the interval $[j^B_t,j^B_{t+1})$
and is in fact at least $ L(j^B_{t+1})$.
The conclusion holds from the following sequence of inequalities,
each of which is easy to see given the discussion so far.
\begin{displaymath}
\RSEM^B(\tfrac{k}{2}) \geq L(j^B_{t+1}) \geq \runder(j^B_{t+1}) \geq
\runder(\tfrac{k}{2})\geq z\IR^A(\tfrac{k}{2})  .
\end{displaymath}

This completes the proof of the lemma.
\end{proof}


Finally, we relate $\IR^A (k/2)$  to the benchmark $\ftwo(k)$ as in the following lemma.
\begin{lemma}\label{lem.sideA}
 $\IR^A (k/2) \geq \frac{s_\lambda}{2\lambda}\cdot \ftwo(k)$.
\end{lemma}

\begin{proof}
In unlimited supply, if the optimum single price sells $\lambda$ units,
i.e. $\ftwo = \lambda \valith[\lambda]$, then
one can offer $\valith[\lambda]$ to the bidders in $A$ and get a revenue of
$\valith[\lambda] s_{\lambda}$, so one would conclude that
\[\f^A  \geq\valith[\lambda] s_{\lambda}= \frac{s_\lambda}{\lambda}\cdot \ftwo.\]
However the same argument does not work in case of limited supply, because
we split the supply also in half for each side.
Thus offering  $\valith[\lambda]$ to the bidders in $A$ is guaranteed to get a revenue of
$ \valith[\lambda]\cdot \min\{ s_{\lambda}, \frac{k}{2}\}.$ Since $s_\lambda \leq k$, we
can use that  $\min\{ s_{\lambda}, \frac{k}{2}\} \geq \frac{s_\lambda}{2}$ to get the required
conclusion for the lemma.
\end{proof}



Our main theorem now follows easily from Lemmas \ref{lem.AMS}, \ref{lem.swap}, \ref{lem.sideA}
and Theorem \ref{thm.benchmarks}.

\begin{theorem}
\label{thm.rsem}
  RSEM is at most a $\min\{8/3, 2(1 + \tfrac{1}{k}) \} \cdot \amscr $-approximation
  with respect to $\f^{(2)}$ and at most a \\$\min\{16/3, 4(1 +\tfrac{1}{k})
  \} \cdot \amscr$-approximation with respect to $\fbar^{(2)}$.\\
 $\frac{16}{3}\cdot\amscr \approx 25$.
\end{theorem}


\paragraph*{Remark}
In using Lemma \ref{lem.AMS} from \cite{AMS-09} as a blackbox, we lose
a factor of 2 in the proof of Lemma \ref{lem.sideA}.  It is natural to
wonder if the random variable $X$ is defined as $z\cdot
\min\{\frac{s_\lambda}{\lambda}, \frac{1}{2} \}$, then what is the
lower bound on $\expect[]X$?  Naively, the bound is
$1/(2\cdot\amscr)$ (as used in the present analysis).
An improvement in this bound would improve the approximation factor in
our analysis.

